Code Recommendation for Open Source Software Developers

Open Source Software (OSS) is forming the spines of technology infrastructures, attracting millions of talents to contribute. Notably, it is challenging and critical to consider both the developers' interests and the semantic features of the project code to recommend appropriate development tasks to OSS developers. In this paper, we formulate the novel problem of code recommendation, whose purpose is to predict the future contribution behaviors of developers given their interaction history, the semantic features of source code, and the hierarchical file structures of projects. Considering the complex interactions among multiple parties within the system, we propose CODER, a novel graph-based code recommendation framework for open source software developers. CODER jointly models microscopic user-code interactions and macroscopic user-project interactions via a heterogeneous graph and further bridges the two levels of information through aggregation on file-structure graphs that reflect the project hierarchy. Moreover, due to the lack of reliable benchmarks, we construct three large-scale datasets to facilitate future research in this direction. Extensive experiments show that our CODER framework achieves superior performance under various experimental settings, including intra-project, cross-project, and cold-start recommendation. We will release all the datasets, code, and utilities for data retrieval upon the acceptance of this work.

==> src/acknowledgements.tex <==



==> src/fig-tsne.tex <==
To further validate the above observation, we randomly sample 10 repositories in the MF dataset and visualize their file embeddings in Fig.~\ref{fig:tsne} using t-SNE~\cite{van2008visualizing}.
A maximum of 300 files are displayed per repository for clarity. 
% The file embeddings are obtained using 4 models: (a) Matrix Factorization~\cite{rendle2009bpr}, (b) LightGCN~\cite{he2020lightgcn}, (c) NCL~\cite{lin2022improving}, and (d) our \model framework.
The file embeddings are obtained using 3 models: (a) LightGCN~\cite{he2020lightgcn}, (b) NCL~\cite{lin2022improving}, and (c) our \model framework.
We observe that models with the contrastive learning objective (NCL and \model) manifest better clustering structures. In particular, file embeddings learned by our \model framework demonstrate the best cross-repository differences. The results further prove that \model jointly models the intra-project and inter-project differences among files, effectively distinguishing the files under the same OSS project, which is more efficient than directly encoding the repository identity in the embedding space.

\begin{figure}
  \centering
  \includegraphics[scale=0.35]{src/img/tsne_v4.pdf}
  \vspace{-2mm}
  % \caption{t-SNE Visualization of the file embeddings on the ML dataset produced by (a) Matrix Factorization; (b) LightGCN; (c) NCL; (d) \model. Files in the same color fall under the same repositories.}
  \caption{t-SNE Visualization of the file embeddings on the ML dataset produced by (a) LightGCN; (b) NCL; (c) \model. Files in the same color fall under the same repositories.}
  \label{fig:tsne}
  \vspace{-5mm}
\end{figure}
